Transformer-based Approach for Accurate Asteroid Spectra taxonomy and albedo estimation

China plans to launch a probe (Tianwen-2) around 2025, mainly for exploring the near-Earth asteroid 2016 HO3 . The mission involves close-range exploration, landing, and mining operations that require three-dimensional modeling of the asteroid, which requires prior knowledge of its material composition and uniformity. This information is crucial in progressive or ground exploration processes. Our research focuses on high-precision intelligent inversion of complex physical properties of asteroids based on spectral data, providing support for further analysis of aster oid materials, density, and structure. We have developed a platform for asteroid spectral classification, albedo estimation, and composition analysis, which includes three types of neural networks based on Transformer attention mechanism: One for spectral classification, achieving a four-class classification accuracy of 97.28% and an eleven-class classification accuracy of 95.69%; second one for albedo estimation, with an average absolute error of 0.0308 in S-type asteroid albedo estimation, and the third one for composition analysis, with a predicted spectral angular distance of only 0.0340 and a root mean square error of 0.1759 for the abundance of end members. These results indicate that our network can provide high-precision asteroid spectral classification, albedo estimation, and composition analysis results. In addition, we utilized the platform to analyze and provide results for six asteroids.

==> bbl.tex <==
\begin{thebibliography}{}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\providecommand{\url}[1]{\href{#1}{#1}}
\providecommand{\dodoi}[1]{doi:~\href{http://doi.org/#1}{\nolinkurl{#1}}}
\providecommand{\doeprint}[1]{\href{http://ascl.net/#1}{\nolinkurl{http://ascl.net/#1}}}
\providecommand{\doarXiv}[1]{\href{https://arxiv.org/abs/#1}{\nolinkurl{https://arxiv.org/abs/#1}}}

\bibitem[{Bin {et~al.}(2023)Bin, Chunlai, Jianjun, Xin, Dawei, Jishi, \& Yan}]{article4}
Bin, L., Chunlai, L., Jianjun, L., {et~al.} 2023, ACTIVE SMALL BODIES IN THE SOLAR SYSTEM OVER A WIDE RANGE OF HELIOCENTRIC DISTANCES, 86

\bibitem[{Bowell {et~al.}(1978)Bowell, Chapman, Gradie, Morrison, \& Zellner}]{bowell1978taxonomy}
Bowell, E., Chapman, C.~R., Gradie, J.~C., Morrison, D., \& Zellner, B. 1978, Icarus, 35, 313

\bibitem[{Bus \& Binzel(2002{\natexlab{a}})}]{article9}
Bus, S.~J., \& Binzel, R.~P. 2002{\natexlab{a}}, Icarus, 158, 106

\bibitem[{Bus \& Binzel(2002{\natexlab{b}})}]{article10}
---. 2002{\natexlab{b}}, Icarus, 158, 146

\bibitem[{Chao {et~al.}(2016)Chao, Yuehua, Haibin, \& Xiaopin}]{article17}
Chao, H., Yuehua, M., Haibin, Z., \& Xiaopin, L. 2016, Acta Astronomica Sinica, 57, 526

\bibitem[{Chapman {et~al.}(1971)Chapman, Johnson, \& McCord}]{article6}
Chapman, C.~R., Johnson, T.~V., \& McCord, T.~B. 1971, 12, 51

\bibitem[{Chapman {et~al.}(1975)Chapman, Morrison, \& Zellner}]{chapman1975surface}
Chapman, C.~R., Morrison, D., \& Zellner, B. 1975, Icarus, 25, 104

\bibitem[{Cheng(2023)}]{article5}
Cheng, M. 2023, Highlights in Science, Engineering and Technology, 48, 295

\bibitem[{Clark(1995)}]{article13}
Clark, B.~E. 1995, Journal of Geophysical Research: Planets, 100, 14443

\bibitem[{De~la Fuente~Marcos \& De~la Fuente~Marcos(2016)}]{article1}
De~la Fuente~Marcos, C., \& De~la Fuente~Marcos, R. 2016, Monthly Notices of the Royal Astronomical Society, 462, 3441

\bibitem[{DeMeo {et~al.}(2015)DeMeo, Alexander, Walsh, Chapman, Binzel, {et~al.}}]{demeo2015compositional}
DeMeo, F., Alexander, C., Walsh, K., {et~al.} 2015, Asteroids iv, 1, 13

\bibitem[{DeMeo {et~al.}(2009)DeMeo, Binzel, Slivan, \& Bus}]{article11}
DeMeo, F.~E., Binzel, R.~P., Slivan, S.~M., \& Bus, S.~J. 2009, Icarus, 202, 160

\bibitem[{Fornasier {et~al.}(2011)Fornasier, Clark, \& Dotto}]{article16}
Fornasier, S., Clark, B.~E., \& Dotto, E. 2011, Icarus, 214, 131

\bibitem[{Gaffey {et~al.}(1993)Gaffey, Bell, Brown, Burbine, Piatek, Reed, \& Chaky}]{article12}
Gaffey, M.~J., Bell, J.~F., Brown, R.~H., {et~al.} 1993, Icarus, 106, 573

\bibitem[{Ghosh {et~al.}(2022)Ghosh, Roy, Koirala, Rasti, \& Scheunders}]{ghosh2022hyperspectral}
Ghosh, P., Roy, S.~K., Koirala, B., Rasti, B., \& Scheunders, P. 2022, IEEE Transactions on Geoscience and Remote Sensing, 60, 1

\bibitem[{Han {et~al.}(2022{\natexlab{a}})Han, Wang, Chen, Chen, Guo, Liu, Tang, Xiao, Xu, Xu, {et~al.}}]{article24}
Han, K., Wang, Y., Chen, H., {et~al.} 2022{\natexlab{a}}, IEEE transactions on pattern analysis and machine intelligence, 45, 87

\bibitem[{Han {et~al.}(2022{\natexlab{b}})Han, Wang, Chen, Chen, Guo, Liu, Tang, Xiao, Xu, Xu, {et~al.}}]{han2022survey}
---. 2022{\natexlab{b}}, IEEE transactions on pattern analysis and machine intelligence, 45, 87

\bibitem[{Hardersen {et~al.}(2011)Hardersen, Cloutis, Reddy, MOTH{\'E}-DINIZ, \& Emery}]{article15}
Hardersen, P.~S., Cloutis, E.~A., Reddy, V., MOTH{\'E}-DINIZ, T., \& Emery, J.~P. 2011, Meteoritics \& Planetary Science, 46, 1910

\bibitem[{Harris(1998)}]{harris1998thermal}
Harris, A.~W. 1998, Icarus, 131, 291

\bibitem[{Heiligers {et~al.}(2019)Heiligers, Fernandez, Stohlman, \& Wilkie}]{article2}
Heiligers, J., Fernandez, J.~M., Stohlman, O.~R., \& Wilkie, W.~K. 2019, Astrodynamics, 3, 231

\bibitem[{Klimczak {et~al.}(2021)Klimczak, Kot{\l}owski, Oszkiewicz, DeMeo, Kryszczy{\'n}ska, Wilawer, \& Carry}]{article18}
Klimczak, H., Kot{\l}owski, W., Oszkiewicz, D., {et~al.} 2021, Frontiers in Astronomy and Space Sciences, 8, 767885

\bibitem[{Korda {et~al.}(2023{\natexlab{a}})Korda, Kohout, Flanderov{\'a}, Vincent, \& Penttil{\"a}}]{article23}
Korda, D., Kohout, T., Flanderov{\'a}, K., Vincent, J.-B., \& Penttil{\"a}, A. 2023{\natexlab{a}}, Astronomy \& Astrophysics, 675, A50

\bibitem[{Korda {et~al.}(2023{\natexlab{b}})Korda, Penttil{\"a}, Klami, \& Kohout}]{article22}
Korda, D., Penttil{\"a}, A., Klami, A., \& Kohout, T. 2023{\natexlab{b}}, Astronomy \& Astrophysics, 669, A101

\bibitem[{Lebofsky \& Spencer(1989)}]{lebofsky1989radiometry}
Lebofsky, L.~A., \& Spencer, J.~R. 1989, Asteroids II, 128

\bibitem[{Lebofsky {et~al.}(1986)Lebofsky, Sykes, Tedesco, Veeder, Matson, Brown, Gradie, Feierberg, \& Rudy}]{lebofsky1986refined}
Lebofsky, L.~A., Sykes, M.~V., Tedesco, E.~F., {et~al.} 1986, Icarus, 68, 239

\bibitem[{LI~Chunlai(2024)}]{sktcxb-11-4-lichunlai}
LI~Chunlai, LIU~Jianjun, R. X. Y. W. Z. Z. L. H. O.~Z. 2024, Journal of Deep Space Exploration, 11, 304, \dodoi{10.15982/j.issn.2096-9287.2024.20230185}

\bibitem[{LING~Honglei(2019)}]{LINGHonglei2019}
LING~Honglei, ZHANG~Xia, Y. Y. G. D. W. X. Q.~W. 2019, Journal of Remote Sensing

\bibitem[{Ling-Zhi {et~al.}(2014)Ling-Zhi, Zong-Cheng, \& Jian-Zhong}]{ling2014spectral}
Ling-Zhi, S., Zong-Cheng, L., \& Jian-Zhong, L. 2014, Earth Science Frontiers, 21, 188

\bibitem[{Lingzhi~Sun(2016)}]{LingzhiSun2016}
Lingzhi~Sun, Zongcheng~Ling, J. Z. B. L. G.~D. 2016, Acta Petrologica Sinica, 32, 43

\bibitem[{Luo {et~al.}(2023)Luo, Wang, Gu, Penttil{\"a}, Muinonen, \& Liu}]{article21}
Luo, N., Wang, X., Gu, S., {et~al.} 2023, The Astronomical Journal, 167, 13

\bibitem[{Mahlke {et~al.}(2022)Mahlke, Carry, \& Mattei}]{article20}
Mahlke, M., Carry, B., \& Mattei, P.-A. 2022, Astronomy \& Astrophysics, 665, A26

\bibitem[{Nakamura {et~al.}(2014)Nakamura, Nakato, Ishida, Wakita, Noguchi, Zolensky, Tanaka, Kimura, Tshuchiyama, Ogami, {et~al.}}]{nakamura2014mineral}
Nakamura, T., Nakato, A., Ishida, H., {et~al.} 2014, Meteoritics \& Planetary Science, 49, 215

\bibitem[{Parente {et~al.}(2011)Parente, Mustard, Murchie, \& Seelos}]{parente2011robust}
Parente, M., Mustard, J.~F., Murchie, S., \& Seelos, F. 2011, in 2011 IEEE International Geoscience and Remote Sensing Symposium, IEEE, 1291--1294

\bibitem[{Penttil{\"a} {et~al.}(2021)Penttil{\"a}, Hietala, \& Muinonen}]{article19}
Penttil{\"a}, A., Hietala, H., \& Muinonen, K. 2021, Astronomy \& Astrophysics, 649, A46

\bibitem[{Potin {et~al.}(2020)Potin, Beck, Usui, Bonal, Vernazza, \& Schmitt}]{article14}
Potin, S., Beck, P., Usui, F., {et~al.} 2020, Icarus, 348, 113826

\bibitem[{Rasti {et~al.}(2022)Rasti, Koirala, \& Scheunders}]{rasti2022hapkecnn}
Rasti, B., Koirala, B., \& Scheunders, P. 2022, IEEE Transactions on Geoscience and Remote Sensing, 60, 1

\bibitem[{Smith(2002)}]{smith2002tutorial}
Smith, L.~I. 2002

\bibitem[{Tholen(1984)}]{article7}
Tholen, D.~J. 1984, Asteroid taxonomy from cluster analysis of photometry (The University of Arizona)

\bibitem[{Tholen \& Barucci(1989)}]{article8}
Tholen, D.~J., \& Barucci, M.~A. 1989, Asteroids II, 298

\bibitem[{Tsuchiyama {et~al.}(2014)Tsuchiyama, Uesugi, Uesugi, Nakano, Noguchi, Matsumoto, Matsuno, Nagano, Imai, Shimada, {et~al.}}]{tsuchiyama2014three}
Tsuchiyama, A., Uesugi, M., Uesugi, K., {et~al.} 2014, Meteoritics \& Planetary Science, 49, 172

\bibitem[{Vaswani {et~al.}(2017)Vaswani, Shazeer, Parmar, Uszkoreit, Jones, Gomez, Kaiser, \& Polosukhin}]{article25}
Vaswani, A., Shazeer, N., Parmar, N., {et~al.} 2017, Advances in neural information processing systems, 30

\bibitem[{Weng {et~al.}(2021)Weng, Lu, \& Yao}]{weng2021one}
Weng, C., Lu, B., \& Yao, J. 2021, in 2021 Global Reliability and Prognostics and Health Management (PHM-Nanjing), IEEE, 1--6

\bibitem[{Yang {et~al.}(2019)Yang, Yang, Yan, Zhang, Zhang, Guo, Sun, \& Fu}]{yang2019scrdet}
Yang, X., Yang, J., Yan, J., {et~al.} 2019, in Proceedings of the IEEE/CVF international conference on computer vision, 8232--8241

\bibitem[{Yin {et~al.}(2019)Yin, Huang, Luo, \& Du}]{yin2019automatic}
Yin, J., Huang, C., Luo, X., \& Du, Q. 2019, Icarus, 319, 349

\bibitem[{Zhang {et~al.}(2019)Zhang, Huang, Wang, \& Huo}]{article3}
Zhang, X., Huang, J., Wang, T., \& Huo, Z. 2019, 1045

\bibitem[{ZHANG~Qi(2016)}]{ZHANGQi2016}
ZHANG~Qi, LIU~Fujiang, L. C. Q. L. G. Z. C.~C. 2016, Remote Sensing for Natural Resources, 7

\end{thebibliography}

